On the Efficiency of Test Suite based Program Repair: A Systematic Assessment of 16 Automated Repair Systems for Java Programs

Test-based automated program repair has been a prolific field of research in software engineering in the last decade. Many approaches have indeed been proposed, which leverage test suites as a weak, but affordable, approximation to program specifications. Although the literature regularly sets new records on the number of benchmark bugs that can be fixed, several studies increasingly raise concerns about the limitations and biases of state-of-the-art approaches. For example, the correctness of generated patches has been questioned in a number of studies, while other researchers pointed out that evaluation schemes may be misleading with respect to the processing of fault localization results. Nevertheless, there is little work addressing the efficiency of patch generation, with regard to the practicality of program repair. In this paper, we fill this gap in the literature, by providing an extensive review on the efficiency of test suite based program repair. Our objective is to assess the number of generated patch candidates, since this information is correlated to (1) the strategy to traverse the search space efficiently in order to select sensical repair attempts, (2) the strategy to minimize the test effort for identifying a plausible patch, (3) as well as the strategy to prioritize the generation of a correct patch. To that end, we perform a large-scale empirical study on the efficiency, in terms of quantity of generated patch candidates of the 16 open-source repair tools for Java programs. The experiments are carefully conducted under the same fault localization configurations to limit biases.

==> tables/NFL_BugTypes.tex <==
\begin{table}[!ht]
	\centering
	\scriptsize
	\caption{Taxonomy of bugs fixed by each APR tool with normal FL.}
%	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{lc}
			\toprule
			{\bf Bug Type} & {\bf bug IDs}\\
			\hline
			Type-1 & Chart-1\\
			Type-2 & Chart-2\\
			\bottomrule
		\end{tabular}
		{$^\ast$Bugs listed in this table are reported as correctly fixed by the corresponding APR tool.}
	\end{threeparttable}
%	}
\end{table}

==> tables/NFL_Details.tex <==
\begin{table}[!ht]
	\centering
	\scriptsize
	\caption{\# of Patches Generated before the generation of the first plausible patch with Normal Fault Localization for jGenProg.}
	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{lccc}
			\toprule
			{\bf Bug ID} & {\bf \# uncompilable patches} & {\bf \# compilable patches} & {\bf Total}\\
			\hline
			Chart-1 & x & y & x + y\\
			Chart-2 & x' & y' & x' + y'\\
			\bottomrule
		\end{tabular}
	\end{threeparttable}
	}
\end{table}

==> tables/NFL_Details2.tex <==
\begin{table}[!ht]
	\centering
	\scriptsize
	\caption{\# of Patches Generated before the generation of the first plausible patch with GZoltar-1.7.3 for jGenProg.}
	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{lccc}
			\toprule
			{\bf Bug ID} & {\bf \# uncompilable patches} & {\bf \# compilable patches} & {\bf Total}\\
			\hline
			Chart-1 & x & y & x + y\\
			Chart-2 & x' & y' & x' + y'\\
			\bottomrule
		\end{tabular}
	\end{threeparttable}
	}
\end{table}

==> tables/NFL_NPC_small.tex <==
\begin{table}[!h]
	\center
	\scriptsize
	\caption{Upper whisker, median and mean values of $NPC$ ($NPC_{in-plausible}$) scores in Figure~\ref{fig:NFL-NPC3}.}
	\label{tab:NFL_NPC}
	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{l|rr|rr|rr|r}
			\toprule
			\multirow{2}{*}{APR Tools} &\multicolumn{2}{c|}{Upper Whisker} & \multicolumn{2}{c|}{Median} & \multicolumn{2}{c|}{Mean} & \multirow{2}{*}{\makecell[c]{\#\\bugs}}\\\cline{2-7}
			& All & Correct & All & Correct  & All & Correct & \\
			\hline
%			jGenProg   & 803 (247) & 191 (79)    & 37 (27) &$\uparrow$ 127 (73)& 670 (436) & 108 (51)\\
%			GenProg-A  & 235 (76)  & 139 (40)    & 34 (10) & 11 (5)  & 187 (81)  & 75 (40)\\
%			jMutRepair &  67 (77)  & 33 (27)     & 17 (13) &$\uparrow$ 28 (13) & 43 (36)  & 32 (27)\\
%			kPAR       &2377 (844) & 992 (383)   &269 (134)&130 (68) & 879 (480) &331 (135)\\
%			RSRepair-A &  208 (65) & 103 (26)    & 34 (10) & 20 (7)  & 250 (81)  & 62 (17)\\
%			jKali      &  92 (83)  & 83 (80)     & 14 (13) & 7 (5)   & 35 (31)   & 30 (28)\\
%			Kali-A     & 43 (38)   & 4 (3)       & 8 (7)   & 2 (1)   & 12 (10)   & 3 (2)\\
%			Dynamoth   & 1 (0)     & 1 (0)       & 1 (0)   & 1 (0)   & 2 (1)     & 1 (0)\\
%			Nopol      & 1 (0)     & 1  (0)      & 1 (0)   & 1 (0)   & 1 (0)     & 1 (0)\\
%			ACS        & 15 (4)    & 11 (3)      & 2 (0)   & 2 (0)   & 15 (4)    &$\uparrow$ 17 (4)\\
%			Cardumen   & 966 (965) & 141 (68)    & 33 (32) & 13 (12) & 479 (454) & 77 (40) \\
%			ARJA       & 362 (302) & $\uparrow$ 686 (648)&30 (19)&$\uparrow$ 87 (83)&142 (117)&$\uparrow$ 195 (184)\\
%			SimFix     &3800 (3799)&2274 (2273)  &163 (162)&168 (167)&1167 (1166)&745 (744)\\
%			FixMiner   & 546 (147) & 357 (99)    &111 (24) & 77 (24) & 754 (189) &609 (81)\\
%			AVATAR     &1624 (512) &$\uparrow$ 2426 (511)&164 (65) &136 (33) &478 (145)&$\uparrow$ 530 (150)\\
%			TBar       &2958 (1262)& 1806 (1031) &220 (117)&102 (48) & 818 (444) &620 (306)\\
			%jGenProg   & 803 (247) & 191 (79)    & 50 (34) &$\uparrow$ 127 (73)& 670 (436) & 108 (51) & 3\\
			%GenProg-A  & 235 (76)  & 139 (40)    & 34 (11) &$\uparrow$ 75 (41)  & 187 (81)  & 75 (40) & 2\\
			%jMutRepair &  67 (77)  & 33 (27)     & 20 (14) &$\uparrow$ 28 (13) & 43 (36)  & 32 (27)   & 5\\
			kPAR       &2377 (844) & 992 (383)   &269 (134)&132 (76) & 879 (480) &331 (135)           & 10\\
			%RSRepair-A &  208 (65) & 103 (26)    & 34 (10) &$\uparrow$ 62 (17)  & 250 (81)  & 62 (17) & 2\\
			%jKali      &  92 (83)  & 83 (80)     & 14 (13) & 7 (5)   & 35 (31)   & 30 (28)            & 3\\
			%Kali-A     & 43 (38)   & 4 (3)       & 8 (7)   & 2 (1)   & 12 (10)   & 3 (2)              & 3\\
			%Dynamoth   & 1 (0)     & 1 (0)       & 1 (0)   & 1 (0)   & 2 (1)     & 1 (0)              & 1\\
			%Nopol      & 1 (0)     & 1  (0)      & 1 (0)   & 1 (0)   & 1 (0)     & 1 (0)              & 2\\
			%ACS        & 15 (4)    & 11 (3)      & 2 (0)   & 2 (0)   & 15 (4)    &$\uparrow$ 17 (4)   & 17\\
			%Cardumen   & 966 (965) & 141 (68)    & 87 (50) & 77 (40) & 479 (454) & 77 (40)            & 2\\
			ARJA       & 362 (302) & $\uparrow$ 686 (648)&38 (22)&$\uparrow$ 136 (116)&142 (117)&$\uparrow$ 195 (184)  & 8\\
			SimFix     &3800 (3799)&2274 (2273)  &166 (165)&307 (306)&1167 (1166)&745 (744)           & 24\\
			FixMiner   & 546 (147) & 357 (99)    &111 (24) & 77 (24) & 754 (189) &609 (81)            & 13\\
			AVATAR     &1624 (512) &$\uparrow$ 2426 (511)&164 (65) &136 (33) &478 (145)&$\uparrow$ 530 (150)&19\\
			TBar       &2958 (1262)& 1806 (1031) &240 (118)&120 (53) & 818 (444) &620 (306)           & 24\\
			\bottomrule
		\end{tabular}
		{$^\ast$The upper whisker value is determined by 1.5 IQR (interquartile ranges) where IQR = 3rd Quartile - 1st Quartile, as defined in~\cite{frigge1989some}.\\
		``All'' denotes all fixed bugs, and ``Correct'' denotes correctly fixed bugs.\\
		The numbers outside the parentheses indicate the related $NPC$ score values and the numbers inside the parentheses indicate the related $NPC_{in-plausible}$ score values.\\
		$\uparrow$ implies that the $NPC$ and $NPC_{in-plausible}$ values of ``Correct'' are higher than those of ``All''.}
	\end{threeparttable}
	}
\end{table}


==> tables/NFL_Results.tex <==
\begin{table}[!ht]
	\centering
	\scriptsize
	\caption{APR Tools' Repair Performance with Normal Fault Localization (i.e., FL tool used in their tools) .}
	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{lccccccc}
			\toprule
			{\bf APR Tool} & {\bf Chart} & {\bf Closure} & {\bf Lang} & {\bf Math} & {\bf Mockito} & {\bf Time} & {\bf Total}\\
			\hline
			jGenProg & x/y & \\
			jKali & \\
			\bottomrule
		\end{tabular}	
		{$^\ast$x: the number of bugs fixed with correct patches, y: the number of bugs fixed with plausible patches.}
	\end{threeparttable}
	}
\end{table}

==> tables/NFL_overlap2.tex <==
\begin{table*}[htbp]
  \scriptsize
  \centering
  \caption{Overlap of correct patches under NFL.}
    \resizebox{\textwidth}{20mm}{
    \begin{tabular}{l|cccccccccccccccc}
    \toprule
          & jGenProg & GenProg-A & jMutRepair & kPAR  & RSRepair-A & jKali & Kali-A & DynaMoth & Nopol & ACS   & Cardumen & ARJA  & SimFix & FixMiner & AVATAR & TBar \\
    \midrule
    jGenProg & 0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (3)} & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (2)} \\
    GenProg-A & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) \\
    jMutRepair & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}40.0\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}60.0\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}60.0\% (3) & \cellcolor[rgb]{ .459,  .443,  .443}60.0\% (3) \\
    kPAR  & \cellcolor[rgb]{ .816,  .808,  .808}10.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}10.0\% (1) & 10.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}10.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}10.0\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (5) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{70.0\% (7)} \\
    RSRepair-A & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) \\
    jKali & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & 0.0\% (0) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (2)} & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (2)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) \\
    Kali-A & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (2)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (2)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (2)} & 0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (3)} & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) \\
    DynaMoth & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (1)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (1)} & 0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (1)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) \\
    Nopol & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 100.0\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) \\
    ACS   & \cellcolor[rgb]{ .816,  .808,  .808}5.9\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}11.8\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}11.8\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 52.9\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}5.9\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}5.9\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}5.9\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}23.5\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}17.6\% (3) \\
    Cardumen & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} \\
    ARJA  & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 37.5\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) \\
    SimFix & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}4.2\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}20.8\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}4.2\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}4.2\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}4.2\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}4.2\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}4.2\% (1) & 41.7\% (10) & \cellcolor[rgb]{ .682,  .667,  .667}20.8\% (5) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}41.7\% (10) \\
    FixMiner & \cellcolor[rgb]{ .816,  .808,  .808}7.7\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}7.7\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}7.7\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}15.4\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & 23.1\% (3) & \cellcolor[rgb]{ .459,  .443,  .443}46.2\% (6) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{76.9\% (10)} \\
    AVATAR & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}5.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}15.8\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}26.3\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}5.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}5.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}5.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}21.1\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}5.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}5.3\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}31.6\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}31.6\% (6) & 21.1\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}57.9\% (11) \\
    TBar  & \cellcolor[rgb]{ .816,  .808,  .808}8.3\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}29.2\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}4.2\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}8.3\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}41.7\% (10) & \cellcolor[rgb]{ .459,  .443,  .443}41.7\% (10) & \cellcolor[rgb]{ .459,  .443,  .443}45.8\% (11) & 29.2\% (7) \\
    \bottomrule
    \end{tabular}}%
  \label{tab:addlabel}%
\end{table*}%

==> tables/PFL_BugTypes.tex <==
\begin{table}[!ht]
	\centering
	\scriptsize
	\caption{Taxonomy of bugs fixed by each APR tool with perfect FL.}
%	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{lc}
			\toprule
			{\bf Bug Type} & {\bf bug IDs}\\
			\hline
			Type-1 & Chart-1\\
			Type-2 & Chart-2\\
			\bottomrule
		\end{tabular}
		{$^\ast$Bugs listed in this table are reported as correctly fixed by the corresponding APR tool.}
	\end{threeparttable}
%	}
\end{table}

==> tables/PFL_Details.tex <==
\begin{table}[!ht]
	\centering
	\scriptsize
	\caption{\# of Patches Generated before the generation of the first plausible patch with Perfect Fault Localization for jGenProg.}
	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{lccc}
			\toprule
			{\bf Bug ID} & {\bf \# uncompilable patches} & {\bf \# compilable patches} & {\bf Total}\\
			\hline
			Chart-1 & x & y & x + y\\
			Chart-2 & x' & y' & x' + y'\\
			\bottomrule
		\end{tabular}
	\end{threeparttable}
	}
\end{table}\include{tables/NFL_NPC}

==> tables/PFL_NPC.tex <==
\begin{table}[!h]
	\center
	\scriptsize
	\caption{Caption.}
	\label{tab:PFL_NPC}
	\begin{threeparttable}
		\begin{tabular}{l|rr|rr|rr}
			\toprule
			\multirow{2}{*}{APR Tools} &\multicolumn{2}{c|}{Upper Whisker} & \multicolumn{2}{c|}{Median} & \multicolumn{2}{c}{Average}\\\cline{2-7}
			& All & Correct & All & Correct  & All & Correct \\
			\hline
%			jGenProg   & 67 & 67 & 15 &$\uparrow$ 19 & 37  & 36\\
%			GenProg-A  & 39 & 39 & 7  &$\uparrow$ 17 & 184 & 19\\
%			jMutRepair & 16 & 14 & 3  & 3  & 11  & 7\\
%			kPAR       & 99 & 38 & 12 & 7  & 70  & 23\\
%			RSRepair-A & 81 & 25 & 12 & 9  & 104 & 91\\
%			jKali      & 2  &$\uparrow$ 8 & 2  & 2 & 3   & $\uparrow$ 5\\
%			Kali-A     & 2  & 2  & 1  &$\uparrow$ 2  & 2   & 2\\
%			Dynamoth   & 1  & 1  & 1  & 1  & 1   & 1\\
%			Nopol      & 1  & 1  & 1  & 1  & 1   & 1\\
%			ACS        & 13 & 10 & 2  & 2  & 6   & 5\\
%			Cardumen   & 7  & 7  & 3  & 1  & 49  & 18\\
%			ARJA       & 31 & 27 & 4  &$\uparrow$ 14 & 32  & 15\\
%			SimFix     & 154& 45 & 16 & 8  & 284 &$\uparrow$ 322\\
%			FixMiner   & 155& 41 & 11 & 6  & 253 & 35\\
%			AVATAR     & 68 & 43 & 12 & 8  & 53  & 19\\
%			TBar       & 167& 45 & 13 & 8  & 76  & 31\\
			jGenProg   & 67 (74) & 67 (54)        & 15 (7)  &$\uparrow$ 19 (11)& 37 (20)   & 36 (23)\\
			GenProg-A  & 39 (34) & 39 (24)        & 7 (2)   &$\uparrow$ 17 (4) & 184 (115) & 19 (8)\\
			jMutRepair & 16 (14) & 14 (13)        & 3 (2)   & 3  (2)& 11 (9)  & 7 (6)\\
			kPAR       & 99 (47) & 38 (21)        & 12 (7)  & 7 (5) & 70 (39) & 23 (18)\\
			RSRepair-A & 81 (42) & 25 (6)         & 12 (3)  & 9 (3) & 104 (52)& 91 (35)\\
			jKali      & 2 (1)   &$\uparrow$ 8 (7)& 2 (1)   & 2 (1) & 3 (2) & $\uparrow$ 5 (4)\\
			Kali-A     & 2 (1)   & 2 (1)          & 1 (0)   &$\uparrow$ 2 (1) & 2 (1) & 2 (1)\\
			Dynamoth   & 1 (0)   & 1  (0)         & 1 (0)   & 1 (0) & 1 (0)   & 1 (0)\\
			Nopol      & 1 (0)   & 1  (0)         & 1 (0)   & 1 (0) & 1 (0)   & 1 (0)\\
			ACS        & 13 (5)  & 10 (4)         & 2 (1)   & 2 (1) & 6 (3)   & 5 (2)\\
			Cardumen   & 7 (6)   & 7 (6)          & 3 (2)   & 1 (0) & 49 (40) & 18 (14) \\
			ARJA       & 31 (42) & 27 (25)        & 4 (2)   &$\uparrow$ 14 (5) & 32 (26)  & 15 (12)\\
			SimFix     &154 (153)& 45 (44)        & 16 (15) & 8 (7) &284 (283)&$\uparrow$ 322 (321)\\
			FixMiner   & 155 (24)& 41 (9)         & 11 (2)  & 6 (2) &253 (136)& 35 (7)\\
			AVATAR     & 68 (20) & 43 (11)        & 12 (3)  & 8 (2) & 53 (16) & 19 (7)\\
			TBar       & 167 (42)& 45 (24)        & 13 (7)  & 8 (4) & 76 (35) & 31 (15)\\
			\bottomrule
		\end{tabular}
		{$^\ast$The upper whisker value is determined by 1.5 IQR (interquartile ranges) where IQR = 3rd Quartile - 1st Quartile, as defined in~\cite{frigge1989some}.}
	\end{threeparttable}
\end{table}

==> tables/PFL_inconsistence.tex <==
\begin{table}[!ht]
	\centering
	\scriptsize
	\caption{APR Tools' Repair Performance with Perfect Fault Localization.}
%	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{lc}
			\toprule
			{\bf Bug ID} & {\bf reason of being failed to fix it}\\
			\hline
			Chart-1 & T\\
			Chart-2 & EX\\
			\bottomrule
		\end{tabular}
		{$^\ast$Bugs listed in this table are reported as correctly/plausibly fixed by the corresponding APR tool.}
	\end{threeparttable}
%	}
\end{table}

==> tables/PFL_overlap.tex <==
%\begin{table*}[htbp]
%  \scriptsize
%  \centering
%  \caption{Overlap under Perfect FL}
%  \label{tab:PFL_overlap}
%  \resizebox{1\textwidth}{!}{
%  \begin{threeparttable}
%    \begin{tabular}{l|cccccccccccccccc}
%    \toprule
%          & ACS   & SimFix & kPar  & Avatar & FixMiner & TBar  & ARJA  & GenProg-A & Kali-A & RSRepair-A & jGenPRog & jKali & Cardumen & jMutRepair & Nopol & DynaMoth \\
%    \midrule
%    ACS   & 39.1\% (9) & \cellcolor[rgb]{ .682,  .667,  .667}26.1\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}39.1\% (9) & \cellcolor[rgb]{ .682,  .667,  .667}39.1\% (9) & \cellcolor[rgb]{ .459,  .443,  .443}43.5\% (10) & \cellcolor[rgb]{ .459,  .443,  .443}47.8\% (11) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}13.0\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}17.4\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}13.0\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}4.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}13.0\% (3) \\
%    SimFix & \cellcolor[rgb]{ .816,  .808,  .808}12.0\% (6) & 12.0\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}56.0\% (28) & \cellcolor[rgb]{ .459,  .443,  .443}48.0\% (24) & \cellcolor[rgb]{ .459,  .443,  .443}56.0\% (28) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.0\% (31)} & \cellcolor[rgb]{ .682,  .667,  .667}30.0\% (15) & \cellcolor[rgb]{ .682,  .667,  .667}26.0\% (13) & \cellcolor[rgb]{ .682,  .667,  .667}30.0\% (15) & \cellcolor[rgb]{ .682,  .667,  .667}32.0\% (16) & \cellcolor[rgb]{ .682,  .667,  .667}22.0\% (11) & \cellcolor[rgb]{ .816,  .808,  .808}12.0\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}18.0\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (10) & \cellcolor[rgb]{ .816,  .808,  .808}8.0\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}10.0\% (5) \\
%    kPar  & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (9) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (28) & 3.2\% (2) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{60.3\% (38)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.9\% (39)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{88.9\% (56)} & \cellcolor[rgb]{ .682,  .667,  .667}25.4\% (16) & \cellcolor[rgb]{ .682,  .667,  .667}20.6\% (13) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (21) & \cellcolor[rgb]{ .682,  .667,  .667}25.4\% (16) & \cellcolor[rgb]{ .816,  .808,  .808}12.7\% (8) & \cellcolor[rgb]{ .816,  .808,  .808}9.5\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}12.7\% (8) & \cellcolor[rgb]{ .816,  .808,  .808}15.9\% (10) & \cellcolor[rgb]{ .816,  .808,  .808}6.3\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (7) \\
%    Avatar & \cellcolor[rgb]{ .816,  .808,  .808}18.0\% (9) & \cellcolor[rgb]{ .459,  .443,  .443}48.0\% (24) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{76.0\% (38)} & 2.0\% (1) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{76.0\% (38)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{92.0\% (46)} & \cellcolor[rgb]{ .682,  .667,  .667}24.0\% (12) & \cellcolor[rgb]{ .682,  .667,  .667}24.0\% (12) & \cellcolor[rgb]{ .682,  .667,  .667}36.0\% (18) & \cellcolor[rgb]{ .682,  .667,  .667}26.0\% (13) & \cellcolor[rgb]{ .816,  .808,  .808}14.0\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}12.0\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}18.0\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (10) & \cellcolor[rgb]{ .816,  .808,  .808}10.0\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}16.0\% (8) \\
%    FixMiner & \cellcolor[rgb]{ .816,  .808,  .808}15.9\% (10) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (28) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.9\% (39)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{60.3\% (38)} & 9.5\% (6) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{76.2\% (48)} & \cellcolor[rgb]{ .682,  .667,  .667}28.6\% (18) & \cellcolor[rgb]{ .682,  .667,  .667}23.8\% (15) & \cellcolor[rgb]{ .682,  .667,  .667}30.2\% (19) & \cellcolor[rgb]{ .682,  .667,  .667}27.0\% (17) & \cellcolor[rgb]{ .816,  .808,  .808}15.9\% (10) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}19.0\% (12) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}7.9\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (9) \\
%    TBar  & \cellcolor[rgb]{ .816,  .808,  .808}12.9\% (11) & \cellcolor[rgb]{ .682,  .667,  .667}36.5\% (31) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{65.9\% (56)} & \cellcolor[rgb]{ .459,  .443,  .443}54.1\% (46) & \cellcolor[rgb]{ .459,  .443,  .443}56.5\% (48) & 10.6\% (9) & \cellcolor[rgb]{ .682,  .667,  .667}21.2\% (18) & \cellcolor[rgb]{ .816,  .808,  .808}18.8\% (16) & \cellcolor[rgb]{ .682,  .667,  .667}25.9\% (22) & \cellcolor[rgb]{ .682,  .667,  .667}22.4\% (19) & \cellcolor[rgb]{ .816,  .808,  .808}11.8\% (10) & \cellcolor[rgb]{ .816,  .808,  .808}5.9\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}14.1\% (12) & \cellcolor[rgb]{ .816,  .808,  .808}10.6\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}5.9\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}8.2\% (7) \\
%    ARJA  & \cellcolor[rgb]{ .816,  .808,  .808}5.6\% (2) & \cellcolor[rgb]{ .459,  .443,  .443}41.7\% (15) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (16) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (12) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (18) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (18) & 2.8\% (1) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (27)} & \cellcolor[rgb]{ .459,  .443,  .443}58.3\% (21) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{88.9\% (32)} & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (12) & \cellcolor[rgb]{ .816,  .808,  .808}19.4\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}16.7\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (8) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (4) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (8) \\
%    GenProg-A & \cellcolor[rgb]{ .816,  .808,  .808}6.9\% (2) & \cellcolor[rgb]{ .459,  .443,  .443}44.8\% (13) & \cellcolor[rgb]{ .459,  .443,  .443}44.8\% (13) & \cellcolor[rgb]{ .459,  .443,  .443}41.4\% (12) & \cellcolor[rgb]{ .459,  .443,  .443}51.7\% (15) & \cellcolor[rgb]{ .459,  .443,  .443}55.2\% (16) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{93.1\% (27)} & 3.4\% (1) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{72.4\% (21)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{96.6\% (28)} & \cellcolor[rgb]{ .682,  .667,  .667}34.5\% (10) & \cellcolor[rgb]{ .682,  .667,  .667}20.7\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}24.1\% (7) & \cellcolor[rgb]{ .682,  .667,  .667}24.1\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}6.9\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}20.7\% (6) \\
%    Kali-A & \cellcolor[rgb]{ .816,  .808,  .808}4.8\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}35.7\% (15) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (21) & \cellcolor[rgb]{ .459,  .443,  .443}42.9\% (18) & \cellcolor[rgb]{ .459,  .443,  .443}45.2\% (19) & \cellcolor[rgb]{ .459,  .443,  .443}52.4\% (22) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (21) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (21) & 21.4\% (9) & \cellcolor[rgb]{ .459,  .443,  .443}52.4\% (22) & \cellcolor[rgb]{ .682,  .667,  .667}21.4\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}19.0\% (8) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}19.0\% (8) & \cellcolor[rgb]{ .816,  .808,  .808}9.5\% (4) & \cellcolor[rgb]{ .682,  .667,  .667}21.4\% (9) \\
%    RSRepair-A & \cellcolor[rgb]{ .816,  .808,  .808}8.8\% (3) & \cellcolor[rgb]{ .459,  .443,  .443}47.1\% (16) & \cellcolor[rgb]{ .459,  .443,  .443}47.1\% (16) & \cellcolor[rgb]{ .682,  .667,  .667}38.2\% (13) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (17) & \cellcolor[rgb]{ .459,  .443,  .443}55.9\% (19) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{94.1\% (32)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{82.4\% (28)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{64.7\% (22)} & 0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}38.2\% (13) & \cellcolor[rgb]{ .682,  .667,  .667}20.6\% (7) & \cellcolor[rgb]{ .682,  .667,  .667}20.6\% (7) & \cellcolor[rgb]{ .682,  .667,  .667}23.5\% (8) & \cellcolor[rgb]{ .816,  .808,  .808}11.8\% (4) & \cellcolor[rgb]{ .682,  .667,  .667}23.5\% (8) \\
%    jGenProg & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (4) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{68.8\% (11)} & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (8) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (10)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (10)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (12)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (10)} & \cellcolor[rgb]{ .459,  .443,  .443}56.3\% (9) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{81.3\% (13)} & 12.5\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}31.3\% (5) \\
%    jKali & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (2) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{87.5\% (7)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (5)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{87.5\% (7)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (8)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{87.5\% (7)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & 0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (3) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (5)} & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (1) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (5)} \\
%    Cardumen & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (2) & \cellcolor[rgb]{ .459,  .443,  .443}56.3\% (9) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (8) & \cellcolor[rgb]{ .459,  .443,  .443}56.3\% (9) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (12)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (12)} & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}18.8\% (3) & 0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}18.8\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (4) \\
%    jMutRepair & \cellcolor[rgb]{ .682,  .667,  .667}27.3\% (3) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{90.9\% (10)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{90.9\% (10)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{90.9\% (10)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{81.8\% (9)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{81.8\% (9)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{72.7\% (8)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{63.6\% (7)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{72.7\% (8)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{72.7\% (8)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{63.6\% (7)} & \cellcolor[rgb]{ .459,  .443,  .443}45.5\% (5) & \cellcolor[rgb]{ .682,  .667,  .667}36.4\% (4) & 0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}18.2\% (2) & \cellcolor[rgb]{ .459,  .443,  .443}45.5\% (5) \\
%    Nopol & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}55.6\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}55.6\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}55.6\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (2) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (2) & 11.1\% (1) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (6)} \\
%    DynaMoth & \cellcolor[rgb]{ .682,  .667,  .667}23.1\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}53.8\% (7) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.5\% (8)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{69.2\% (9)} & \cellcolor[rgb]{ .459,  .443,  .443}53.8\% (7) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.5\% (8)} & \cellcolor[rgb]{ .459,  .443,  .443}46.2\% (6) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{69.2\% (9)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.5\% (8)} & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & \cellcolor[rgb]{ .682,  .667,  .667}30.8\% (4) & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}46.2\% (6) & 7.7\% (1) \\
%    \bottomrule
%    \end{tabular}%
%    \end{threeparttable}
%    }
%  \label{tab:addlabel}%
%\end{table*}%



\begin{table*}[htbp]
  \scriptsize
  \centering
  \caption{Overlap of plausible patches under PFL.}
  \resizebox{\textwidth}{20mm}{
    \begin{tabular}{l|cccccccccccccccc}
    \toprule
          & jGenProg & GenProg-A & jMutRepair & kPAR  & RSRepair-A & jKali & Kali-A & DynaMoth & Nopol & ACS   & Cardumen & ARJA  & SimFix & FixMiner & AVATAR & TBar \\
\cmidrule{2-17}    jGenProg & 12.5\% (2) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (10)} & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (8) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{81.3\% (13)} & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}56.3\% (9) & \cellcolor[rgb]{ .682,  .667,  .667}31.3\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (12)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{68.8\% (11)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (10)} & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (10)} \\
    GenProg-A & \cellcolor[rgb]{ .682,  .667,  .667}34.5\% (10) & 3.4\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}24.1\% (7) & \cellcolor[rgb]{ .459,  .443,  .443}44.8\% (13) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{96.6\% (28)} & \cellcolor[rgb]{ .682,  .667,  .667}20.7\% (6) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{72.4\% (21)} & \cellcolor[rgb]{ .682,  .667,  .667}20.7\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}6.9\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}6.9\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}24.1\% (7) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{93.1\% (27)} & \cellcolor[rgb]{ .459,  .443,  .443}44.8\% (13) & \cellcolor[rgb]{ .459,  .443,  .443}51.7\% (15) & \cellcolor[rgb]{ .459,  .443,  .443}41.4\% (12) & \cellcolor[rgb]{ .459,  .443,  .443}55.2\% (16) \\
    jMutRepair & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{63.6\% (7)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{63.6\% (7)} & 0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{90.9\% (10)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{72.7\% (8)} & \cellcolor[rgb]{ .459,  .443,  .443}45.5\% (5) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{72.7\% (8)} & \cellcolor[rgb]{ .459,  .443,  .443}45.5\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}18.2\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}27.3\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}36.4\% (4) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{72.7\% (8)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{90.9\% (10)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{81.8\% (9)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{90.9\% (10)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{81.8\% (9)} \\
    kPAR  & \cellcolor[rgb]{ .816,  .808,  .808}12.7\% (8) & \cellcolor[rgb]{ .682,  .667,  .667}20.6\% (13) & \cellcolor[rgb]{ .816,  .808,  .808}15.9\% (10) & 3.2\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}25.4\% (16) & \cellcolor[rgb]{ .816,  .808,  .808}9.5\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (21) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}6.3\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}12.7\% (8) & \cellcolor[rgb]{ .682,  .667,  .667}25.4\% (16) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (28) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.9\% (39)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{60.3\% (38)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{88.9\% (56)} \\
    RSRepair-A & \cellcolor[rgb]{ .682,  .667,  .667}38.2\% (13) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{82.4\% (28)} & \cellcolor[rgb]{ .682,  .667,  .667}23.5\% (8) & \cellcolor[rgb]{ .459,  .443,  .443}47.1\% (16) & 0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}20.6\% (7) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{64.7\% (22)} & \cellcolor[rgb]{ .682,  .667,  .667}23.5\% (8) & \cellcolor[rgb]{ .816,  .808,  .808}11.8\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}8.8\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}20.6\% (7) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{94.1\% (32)} & \cellcolor[rgb]{ .459,  .443,  .443}47.1\% (16) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (17) & \cellcolor[rgb]{ .682,  .667,  .667}38.2\% (13) & \cellcolor[rgb]{ .459,  .443,  .443}55.9\% (19) \\
    jKali & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (5)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{87.5\% (7)} & 0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (8)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (5)} & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (3) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{87.5\% (7)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{87.5\% (7)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (6)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.5\% (5)} \\
    Kali-A & \cellcolor[rgb]{ .682,  .667,  .667}21.4\% (9) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (21) & \cellcolor[rgb]{ .816,  .808,  .808}19.0\% (8) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (21) & \cellcolor[rgb]{ .459,  .443,  .443}52.4\% (22) & \cellcolor[rgb]{ .816,  .808,  .808}19.0\% (8) & 21.4\% (9) & \cellcolor[rgb]{ .682,  .667,  .667}21.4\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}9.5\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}4.8\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (21) & \cellcolor[rgb]{ .682,  .667,  .667}35.7\% (15) & \cellcolor[rgb]{ .459,  .443,  .443}45.2\% (19) & \cellcolor[rgb]{ .459,  .443,  .443}42.9\% (18) & \cellcolor[rgb]{ .459,  .443,  .443}52.4\% (22) \\
    DynaMoth & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}46.2\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}53.8\% (7) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.5\% (8)} & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{69.2\% (9)} & 7.7\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}46.2\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}23.1\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}30.8\% (4) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.5\% (8)} & \cellcolor[rgb]{ .682,  .667,  .667}38.5\% (5) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{69.2\% (9)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.5\% (8)} & \cellcolor[rgb]{ .459,  .443,  .443}53.8\% (7) \\
    Nopol & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (2) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (6)} & 11.1\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (3) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}55.6\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}55.6\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}55.6\% (5) \\
    ACS   & \cellcolor[rgb]{ .816,  .808,  .808}17.4\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}13.0\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}39.1\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}13.0\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}13.0\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}4.3\% (1) & 39.1\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}8.7\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}26.1\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}43.5\% (10) & \cellcolor[rgb]{ .682,  .667,  .667}39.1\% (9) & \cellcolor[rgb]{ .459,  .443,  .443}47.8\% (11) \\
    Cardumen & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (8) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}18.8\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}18.8\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (2) & 0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}56.3\% (9) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (12)} & \cellcolor[rgb]{ .459,  .443,  .443}56.3\% (9) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (12)} \\
    ARJA  & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (12) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{75.0\% (27)} & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (8) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (16) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{88.9\% (32)} & \cellcolor[rgb]{ .816,  .808,  .808}19.4\% (7) & \cellcolor[rgb]{ .459,  .443,  .443}58.3\% (21) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (8) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}5.6\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}16.7\% (6) & 2.8\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}41.7\% (15) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (18) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (12) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (18) \\
    SimFix & \cellcolor[rgb]{ .682,  .667,  .667}22.0\% (11) & \cellcolor[rgb]{ .682,  .667,  .667}26.0\% (13) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (10) & \cellcolor[rgb]{ .459,  .443,  .443}56.0\% (28) & \cellcolor[rgb]{ .682,  .667,  .667}32.0\% (16) & \cellcolor[rgb]{ .816,  .808,  .808}12.0\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}30.0\% (15) & \cellcolor[rgb]{ .816,  .808,  .808}10.0\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}8.0\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}12.0\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}18.0\% (9) & \cellcolor[rgb]{ .682,  .667,  .667}30.0\% (15) & 12.0\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}56.0\% (28) & \cellcolor[rgb]{ .459,  .443,  .443}48.0\% (24) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{62.0\% (31)} \\
    FixMiner & \cellcolor[rgb]{ .816,  .808,  .808}15.9\% (10) & \cellcolor[rgb]{ .682,  .667,  .667}23.8\% (15) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (9) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{61.9\% (39)} & \cellcolor[rgb]{ .682,  .667,  .667}27.0\% (17) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (7) & \cellcolor[rgb]{ .682,  .667,  .667}30.2\% (19) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}7.9\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}15.9\% (10) & \cellcolor[rgb]{ .816,  .808,  .808}19.0\% (12) & \cellcolor[rgb]{ .682,  .667,  .667}28.6\% (18) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (28) & 9.5\% (6) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{60.3\% (38)} & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{76.2\% (48)} \\
    AVATAR & \cellcolor[rgb]{ .816,  .808,  .808}14.0\% (7) & \cellcolor[rgb]{ .682,  .667,  .667}24.0\% (12) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (10) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{76.0\% (38)} & \cellcolor[rgb]{ .682,  .667,  .667}26.0\% (13) & \cellcolor[rgb]{ .816,  .808,  .808}12.0\% (6) & \cellcolor[rgb]{ .682,  .667,  .667}36.0\% (18) & \cellcolor[rgb]{ .816,  .808,  .808}16.0\% (8) & \cellcolor[rgb]{ .816,  .808,  .808}10.0\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}18.0\% (9) & \cellcolor[rgb]{ .816,  .808,  .808}18.0\% (9) & \cellcolor[rgb]{ .682,  .667,  .667}24.0\% (12) & \cellcolor[rgb]{ .459,  .443,  .443}48.0\% (24) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{76.0\% (38)} & 2.0\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{92.0\% (46)} \\
    TBar  & \cellcolor[rgb]{ .816,  .808,  .808}11.8\% (10) & \cellcolor[rgb]{ .816,  .808,  .808}18.8\% (16) & \cellcolor[rgb]{ .816,  .808,  .808}10.6\% (9) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{65.9\% (56)} & \cellcolor[rgb]{ .682,  .667,  .667}22.4\% (19) & \cellcolor[rgb]{ .816,  .808,  .808}5.9\% (5) & \cellcolor[rgb]{ .682,  .667,  .667}25.9\% (22) & \cellcolor[rgb]{ .816,  .808,  .808}8.2\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}5.9\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}12.9\% (11) & \cellcolor[rgb]{ .816,  .808,  .808}14.1\% (12) & \cellcolor[rgb]{ .682,  .667,  .667}21.2\% (18) & \cellcolor[rgb]{ .682,  .667,  .667}36.5\% (31) & \cellcolor[rgb]{ .459,  .443,  .443}56.5\% (48) & \cellcolor[rgb]{ .459,  .443,  .443}54.1\% (46) & 10.6\% (9) \\
    \bottomrule
    \end{tabular}}%
  \label{tab:addlabel}%
\end{table*}%

==> tables/PFL_overlap2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \scriptsize
  \centering
  \caption{Overlap of correct patches under PFL}
  \resizebox{\textwidth}{20mm}{
    \begin{tabular}{l|cccccccccccccccc}
    \toprule
          & jGenProg & GenProg-A & jMutRepair & kPAR  & RSRepair-A & jKali & Kali-A & DynaMoth & Nopol & ACS   & Cardumen & ARJA  & SimFix & FixMiner & AVATAR & TBar \\
    \midrule
    jGenProg & 14.3\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}42.9\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{71.4\% (5)} & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}28.6\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{71.4\% (5)} & \cellcolor[rgb]{ .459,  .443,  .443}42.9\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}28.6\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}42.9\% (3) \\
    GenProg-A & \cellcolor[rgb]{ .459,  .443,  .443}42.9\% (3) & 0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{85.7\% (6)} & \cellcolor[rgb]{ .682,  .667,  .667}28.6\% (2) & \cellcolor[rgb]{ .459,  .443,  .443}42.9\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{85.7\% (6)} & \cellcolor[rgb]{ .682,  .667,  .667}28.6\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}28.6\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}28.6\% (2) \\
    jMutRepair & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}60.0\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}40.0\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}60.0\% (3) & \cellcolor[rgb]{ .459,  .443,  .443}60.0\% (3) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (5)} & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (5)} \\
    kPAR  & \cellcolor[rgb]{ .816,  .808,  .808}3.8\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}3.8\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}11.5\% (3) & 0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}7.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}23.1\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}7.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}7.7\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}23.1\% (6) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{65.4\% (17)} & \cellcolor[rgb]{ .459,  .443,  .443}57.7\% (15) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (26)} \\
    RSRepair-A & \cellcolor[rgb]{ .459,  .443,  .443}55.6\% (5) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (6)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (2) & 0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{88.9\% (8)} & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}11.1\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}22.2\% (2) & \cellcolor[rgb]{ .459,  .443,  .443}44.4\% (4) \\
    jKali & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & 0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) \\
    Kali-A & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (2) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (2) & 16.7\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}16.7\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}16.7\% (1) \\
    DynaMoth & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (2)} & 0.0\% (0) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{66.7\% (2)} & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}33.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) \\
    Nopol & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{100.0\% (2)} & 0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .459,  .443,  .443}50.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) \\
    ACS   & \cellcolor[rgb]{ .816,  .808,  .808}6.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}6.3\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 37.5\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}12.5\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}31.3\% (5) & \cellcolor[rgb]{ .682,  .667,  .667}37.5\% (6) & \cellcolor[rgb]{ .459,  .443,  .443}43.8\% (7) \\
    Cardumen & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}40.0\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & 20.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}20.0\% (1) & \cellcolor[rgb]{ .459,  .443,  .443}60.0\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}40.0\% (2) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{80.0\% (4)} \\
    ARJA  & \cellcolor[rgb]{ .459,  .443,  .443}45.5\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}54.5\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}18.2\% (2) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{72.7\% (8)} & \cellcolor[rgb]{ .816,  .808,  .808}18.2\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}27.3\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}9.1\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}9.1\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}9.1\% (1) & 0.0\% (0) & \cellcolor[rgb]{ .682,  .667,  .667}27.3\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}27.3\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}18.2\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}36.4\% (4) \\
    SimFix & \cellcolor[rgb]{ .816,  .808,  .808}10.3\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}6.9\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}10.3\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}20.7\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}10.3\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}6.9\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}3.4\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}10.3\% (3) & 27.6\% (8) & \cellcolor[rgb]{ .682,  .667,  .667}34.5\% (10) & \cellcolor[rgb]{ .682,  .667,  .667}27.6\% (8) & \cellcolor[rgb]{ .459,  .443,  .443}51.7\% (15) \\
    FixMiner & \cellcolor[rgb]{ .816,  .808,  .808}5.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}2.9\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}8.6\% (3) & \cellcolor[rgb]{ .459,  .443,  .443}48.6\% (17) & \cellcolor[rgb]{ .816,  .808,  .808}2.9\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}14.3\% (5) & \cellcolor[rgb]{ .816,  .808,  .808}8.6\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}8.6\% (3) & \cellcolor[rgb]{ .682,  .667,  .667}28.6\% (10) & 11.4\% (4) & \cellcolor[rgb]{ .459,  .443,  .443}60.0\% (21) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{80.0\% (28)} \\
    AVATAR & \cellcolor[rgb]{ .816,  .808,  .808}3.1\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}6.3\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}15.6\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}46.9\% (15) & \cellcolor[rgb]{ .816,  .808,  .808}6.3\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}6.3\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}9.4\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}18.8\% (6) & \cellcolor[rgb]{ .816,  .808,  .808}6.3\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}6.3\% (2) & \cellcolor[rgb]{ .682,  .667,  .667}25.0\% (8) & \cellcolor[rgb]{ .227,  .22,  .22}\textcolor[rgb]{ 1,  1,  1}{65.6\% (21)} & 3.1\% (1) & \cellcolor[rgb]{ .051,  .051,  .051}\textcolor[rgb]{ 1,  1,  1}{81.3\% (26)} \\
    TBar  & \cellcolor[rgb]{ .816,  .808,  .808}5.6\% (3) & \cellcolor[rgb]{ .816,  .808,  .808}3.7\% (2) & \cellcolor[rgb]{ .816,  .808,  .808}9.3\% (5) & \cellcolor[rgb]{ .459,  .443,  .443}48.1\% (26) & \cellcolor[rgb]{ .816,  .808,  .808}7.4\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}1.9\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}1.9\% (1) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}0.0\% (0) & \cellcolor[rgb]{ .816,  .808,  .808}13.0\% (7) & \cellcolor[rgb]{ .816,  .808,  .808}7.4\% (4) & \cellcolor[rgb]{ .816,  .808,  .808}7.4\% (4) & \cellcolor[rgb]{ .682,  .667,  .667}27.8\% (15) & \cellcolor[rgb]{ .459,  .443,  .443}51.9\% (28) & \cellcolor[rgb]{ .459,  .443,  .443}48.1\% (26) & 14.8\% (8) \\
    \bottomrule
    \end{tabular}}%
  \label{tab:addlabel}%
\end{table*}%

